Pop-Out Motion: 3D-Aware Image Deformation via Learning the Shape Laplacian

We propose a framework that can deform an object in a 2D image as it exists in 3D space. Most existing methods for 3D-aware image manipulation are limited to (1) only changing the global scene information or depth, or (2) manipulating an object of specific categories. In this paper, we present a 3D-aware image deformation method with minimal restrictions on shape category and deformation type. While our framework leverages 2D-to-3D reconstruction, we argue that reconstruction is not sufficient for realistic deformations due to the vulnerability to topological errors. Thus, we propose to take a supervised learning-based approach to predict the shape Laplacian of the underlying volume of a 3D reconstruction represented as a point cloud. Given the deformation energy calculated using the predicted shape Laplacian and user-defined deformation handles (e.g., keypoints), we obtain bounded biharmonic weights to model plausible handle-based image deformation. In the experiments, we present our results of deforming 2D character and clothed human images. We also quantitatively show that our approach can produce more accurate deformation weights compared to alternative methods (i.e., mesh reconstruction and point cloud Laplacian methods).

==> header.tex <==
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{marvosym}
\usepackage{capt-of}
\usepackage[accsupp]{axessibility}
\usepackage{multicol}
\usepackage{blindtext}


\newcolumntype{Y}{>{\centering\arraybackslash}X}

\usepackage{stackengine}
\def\cross{%
  \stackon[1ex]{\rule{0.4pt}{1.5ex}}{\rule{.75ex}{0.4pt}}}
\def\invcross{%
  \stackon[0.5ex]{\rule{0.4pt}{1.5ex}}{\rule{.75ex}{0.4pt}}}
\def\stacktype{L}

% \definecolor{color_1}{RGB}{255,0,128}
% \definecolor{color_2}{RGB}{0,128,128}
% \definecolor{color_3}{RGB}{0,128,0}
% \definecolor{color_4}{RGB}{128,0,0}

% \newcommand\Minhyuk[1] {\emph{\textcolor{color_1}{Minhyuk: #1}}}
% \newcommand\Jihyun[1] {\emph{\textcolor{color_2}{Jihyun: #1}}}
% \newcommand\Hyunjin[1] {\emph{\textcolor{color_3}{Hyunjin: #1}}}
% \newcommand\Taekyun[1] {\emph{\textcolor{color_4}{Taekyun: #1}}}

==> latex/figures/figure_rebuttal.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{latex/figures/rebuttal_fig.png}
\vspace{-0.6cm}
\caption{\textbf{Comparisons with ``PCD Laplacian'' (best viewed with 200\% zoom-in).} Learned deformation weights are visualized via color-coding. Red spheres indicate the control points.}
\vspace{-0.6cm}
\label{fig:pcd_comparison}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> latex/tables/table_ablation_ap.tex <==
\begin{table}[!h]
\centering
{ \small
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{Point Pair Sampling Strategy ablation.} $\mathrm{PPSS}$ denotes our point pair sampling strategy for Cotangent Laplacian Prediction Module -- as discussed in Section \ref{subsubsec:laplacian_learning_network}. All experimental setups are the same as in the DFAUST experiments in the main paper (refer to Section \textcolor{red}{4.4}). We use 16 point handles selected via farthest point sampling.}
\label{table:ablation_study_ap}

\begin{tabularx}{\columnwidth}{>{\centering}m{2.8cm}|YYYY}
\toprule
Metric &
w/o $\mathrm{PPSS}$ &
w/ $\mathrm{PPSS}$ (Ours) \\

\midrule
Weight L1 ($\times$100) $\downarrow$ & 2.79 & \textbf{2.10} \\
Shape CD ($\times$100) $\downarrow$ & 2.46 & \textbf{1.81} \\
Shape HD ($\times$0.1) $\downarrow$ & 0.43 & \textbf{0.42} \\

\bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\end{table}


% \begin{table}[!h]
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% Metric & \begin{tabular}[c]{@{}c@{}} Our Method\end{tabular} & \begin{tabular}[c]{@{}c@{}}$-\alpha$ \end{tabular} & \begin{tabular}[c]{@{}c@{}} $\mathrm{EM\; Only}$ \end{tabular} & \begin{tabular}[c]{@{}c@{}} $\mathrm{AD\; Only}$ \end{tabular}  \\ \midrule
% Weight L1 ($\times$ 100) $\downarrow$ &  \textbf{2.10} & 4.95 & 3.54 & 2.35   \\ \cmidrule(l){1-5} Shape CD ($\times$ 100) $\downarrow$ & \textbf{1.81} & 4.07 & 3.27 & 2.20\\ \cmidrule(l){1-5} Shape HD ($\times$ 0.1) $\downarrow$ & \textbf{0.42} & 1.23 & 0.69 & 0.47 \\  \bottomrule
% \end{tabular}}
% \end{center}
% \vspace{-0.5cm}
% \caption{\textbf{Ablation studies.} $-\alpha$ indicates a setting where the weight function $\alpha$ is removed from our Laplacian Learning Network. $\mathrm{EM\; Only}$ and $\mathrm{AD\; Only}$ denote settings where $\gamma_1$ and $\gamma_2$ are both instantiated as element-wise multiplication and absolute difference, respectively. All the other experimental setups (e.g., datasets, control handle configurations) are the same as in the target-driven deformation experiment in Section \ref{subsec:3d_point_cloud_deformation}.}
% \label{table:ablation_study}
% \end{table}



==> latex/tables/table_faust.tex <==
\begin{table*}[!t]
\centering
{ \footnotesize
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{Quantitative comparison of point cloud deformation results on FAUST dataset.} The point handles for a source shape are selected using farthest point sampling.}
\label{table:dfaust_results}
\begin{tabularx}{\textwidth}{>{\centering}m{2.5cm}|>{\centering}m{2.8cm}|YYYYYY}
\toprule
Number of Handles &
Metric &

PSR \cite{kazhdan2013screened} &
APSS  \cite{apss} &
BPA \cite{bernardini1999ball} &
DeepSDF \cite{park2019deepsdf} &
DGP \cite{williams2019deep}& Ours \\

\midrule
\multirow{3}{*}{16} & Weight L1 ($\times$100) $\downarrow$ & 3.86 & 3.46 & 4.32 & 2.66 & 4.15 & \textbf{2.10} \\
& Shape CD ($\times$100) $\downarrow$ & 3.84 & 3.04 & 3.83 & 2.61 & 4.09 & \textbf{1.81} \\
& Shape HD ($\times$0.1) $\downarrow$ & 1.81 & 1.31 & 1.73 & 0.48 & 2.85 & \textbf{0.42} \\
 
\midrule
\multirow{3}{*}{32} & Weight L1 ($\times$100) $\downarrow$  & 3.08 & 1.53 & 1.72 & 1.38 & 3.01 & \textbf{1.06} \\
& Shape CD ($\times$100) $\downarrow$ & 5.12 & 2.39 & 2.29 & 2.15 & 4.55  & \textbf{1.45} \\
& Shape HD ($\times$0.1) $\downarrow$  & 3.39 & 0.79 & 0.83  & 0.57 & 4.25 & \textbf{0.53}\\                                                  

\bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[!t]
% \begin{center}
% %\resizebox{1.9\columnwidth}{!}{
% { \small
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% Number of Handles          & Metric & \begin{tabular}[c]{@{}c@{}}Our Method\end{tabular} & \begin{tabular}[c]{@{}c@{}}PSR \cite{kazhdan2013screened} \end{tabular} & \begin{tabular}[c]{@{}c@{}} APSS  \cite{apss}\end{tabular} & \begin{tabular}[c]{@{}c@{}}BPA \cite{bernardini1999ball} \end{tabular} & DeepSDF \cite{park2019deepsdf} & \begin{tabular}[c]{@{}c@{}}DGP \cite{williams2019deep}\end{tabular} \\ \midrule
% \multirow{4}{*}{16}  & Weight L1 ($\times$ 100) $\downarrow$ &  \textbf{2.10} & 3.86 & 3.46 & 4.32 & 2.66 & 4.15                                                                      &            &            \\ \cmidrule(l){2-10} & Shape CD ($\times$ 100) $\downarrow$ & \textbf{1.81} & 3.84 & 3.04 & 3.83 & 2.61               &    4.09                                                                   &            &            \\ \cmidrule(l){2-10} & Shape HD ($\times$ 0.1) $\downarrow$ & \textbf{0.42} & 1.81 & 1.31 & 1.73 & 0.48 & 2.85                                                                      &            &            \\  \midrule
%                          \multirow{4}{*}{32}  & Weight L1 ($\times$ 100) $\downarrow$ & \textbf{1.06}  & 3.08 & 1.53 & 1.72 &    1.38            & 3.01                                                                      &            &            \\ \cmidrule(l){2-10} & Shape CD ($\times$ 100) $\downarrow$ & \textbf{1.45} & 5.12 & 2.39 & 2.29 & 2.15 & 4.55                                                                      &            &            \\ \cmidrule(l){2-10} & Shape HD ($\times$ 0.1) $\downarrow$ & \textbf{0.53} & 3.39 & 0.79 & 0.83  & 0.57 & 4.25                                                                      &            &            \\ \bottomrule
% \end{tabular}}
% \end{center}
% \vspace{-0.5cm}
% \caption{\textbf{Quantitative comparison of target-driven deformation results on DFAUST dataset.} The point handles for a source shape are selected using farthest point sampling.}
% \label{table:dfaust_results}
% \end{table*}
